Autoencoder-Based and Physically Motivated Koopman Lifted States for Wind Farm MPC: A Comparative Case Study

This paper explores the use of Autoencoder (AE) models to identify Koopman-based linear representations for designing model predictive control (MPC) for wind farms. Wake interactions in wind farms are challenging to model, previously addressed with Koopman lifted states. In this study we investigate the performance of two AE models: The first AE model estimates the wind speeds acting on the turbines these are affected by changes in turbine control inputs. The wind speeds estimated by this AE model are then used in a second step to calculate the power output via a simple turbine model based on physical equations. The second AE model directly estimates the wind farm output, i.e., both turbine and wake dynamics are modeled. The primary inquiry of this study addresses whether any of these two AE-based models can surpass previously identified Koopman models based on physically motivated lifted states. We find that the first AE model, which estimates the wind speed and hence includes the wake dynamics, but excludes the turbine dynamics outperforms the existing physically motivated Koopman model. However, the second AE model, which estimates the farm power directly, underperforms when the turbines' underlying physical assumptions are correct. We additionally investigate specific conditions under which the second, purely data-driven AE model can excel: Notably, when modeling assumptions, such as the wind turbine power coefficient, are erroneous and remain unchecked within the MPC controller. In such cases, the data-driven AE models, when updated with recent data reflecting changed system dynamics, can outperform physics-based models operating under outdated assumptions.

==> 1Introduction.tex <==
\section{Introduction}

Model Predictive Control (MPC) is a powerful technique for controlling nonlinear systems with time-varying parameters. However, its effectiveness relies on accurate models of the system dynamics, which can be challenging to obtain, especially for complex systems like wind farms, power grids, and autonomous vehicles. To address this challenge, researchers have turned to the Koopman operator \cite{koopman1931hamiltonian}, a mathematical tool that provides a linear representation of nonlinear dynamical systems.

In recent years, the integration of deep learning techniques with Koopman theory has shown promise in learning the dynamics of nonlinear systems. This approach leverages neural networks, particularly autoencoders, to extract essential features from high-dimensional data, enabling the development of accurate system models. Notably, \cite{lusch2018deep} proposed modifying autoencoders to learn Koopman eigenfunctions parameterized by the continuous frequency of unforced systems.

Several studies have explored the application of deep Koopman models in various domains. For instance, \cite{ping2021deep} introduced a deep Koopman model predictive control approach to enhance transient stability in power grids, employing a network architecture with a nonlinear encoder and linear matrices $A$ and $B$, with $C$ calculated using Dynamic Mode Decomposition (DMD). Similarly, \cite{iacob2021deep} utilized deep neural networks with Koopman operators for system identification, focusing on learning the dynamics of nonlinear systems from data.

In the domain of autonomous vehicles, \cite{xiao2022deep} investigated the application of deep Koopman operators for modeling and control, featuring a network architecture with a nonlinear encoder and linear matrices $A$ and $B$, augmented with true states to form an identity matrix $C$. Likewise, \cite{shi2022deep} employed deep Koopman operators for controlling nonlinear systems, introducing an auxiliary control network to model state-dependent nonlinearity in control input.

Specifically in wind farm control, \cite{chen2022model} presented a nonlinear MPC approach based on deep learning-based reduced-order modeling. The network architecture included a nonlinear encoder and linear matrices $A$ and $B$, with a nonlinear decoder, and they designed another network for power prediction which includes parameter varying C, D, and offset term. The control strategy involves nonlinear MPC, but concerns exist regarding real-time capability due to the requirement for numerous measurement points during identification and control. 
%In another study by \cite{iacob2021deep}, deep neural networks with Koopman operators are used for system identification. The network architecture includes a nonlinear encoder and linear matrices A and B, with C determined using the deepSI toolbox. This study focuses solely on system identification, aiming to learn the dynamics of nonlinear systems from data.
%
%The paper by \cite{xiao2022deep} explores the application of deep Koopman operators in modeling and controlling autonomous vehicles. The network architecture features a nonlinear encoder and linear matrices A and B, with lifted states augmented with true states, resulting in an identity matrix C. The control strategy involves MPC with augmented state space, leveraging the learned system dynamics for control.
%
%Similarly, in the study by \cite{shi2022deep}, deep Koopman operators are employed for controlling nonlinear systems. The network architecture comprises a nonlinear encoder and linear matrices A and B, with lifted states augmented with true states, leading to an identity matrix C. An auxiliary control network is introduced to model state-dependent nonlinearity in control input, enhancing prediction performance to apply linear control methods like Linear Quadratic Regulator.
%In summary, the integration of deep learning techniques with Koopman theory holds significant potential for modeling and controlling complex nonlinear systems.
%
%In the context of wind farm control, the paper \cite{chen2022model} on wind farm power tracking with deep learning-based reduced-order modeling presents a nonlinear MPC approach based on deep learning-based reduced-order modeling. The network architecture for state prediction includes a nonlinear encoder and linear matrices A and B, with a nonlinear decoder, and they designed another network for power prediction which includes parameter varying C, D, and offset term. The control strategy involves nonlinear MPC, but concerns exist regarding real-time capability due to the requirement for numerous measurement points during identification and control. 

%Further, the comparison of the number of measurements required for identification and control in existing and proposed Koopman-based wind farm control is tabulated in Table ~\ref{tab:WFModels}. Here WRC and AIC denote wake redirection and axial induction control respectively.
%The controllers highlighted in dark blue and light blue color are from TU Delft and our previous work respectively.
%In our previous work, we also identified the Koopman model of wind farm and controlled the farm power using quasi-linear MPC (qlMPC) or Koopman MPC (KMPC). However, the Koopman-lifted states were motivated by the physics behind the wakes and turbine models. The controller highlighted in yellow color uses autoencoder and designed by \cite{chen2022model}. Controllers highlighted in green color are the proposed controllers in this work. The table summarizes the measurements required to design the controller in AIC(AE1) are same as required in our previous work that also required less measurements in comparison to other existing literature. Moreover, the AIC(AE2) requires even fewer measurements (only turbine power) for identification and control. 
The comparison of measurement requirements for identification and control in both existing and proposed Koopman-based wind farm control approaches is presented in Table ~\ref{tab:WFModels}. Here, WRC and AIC denote wake redirection and axial induction control, respectively. Controllers highlighted in dark blue and light blue represent those from TU Delft and our previous work, respectively.

In our prior research, we identified the Koopman model of wind farms and controlled farm power using quasi-linear MPC (qlMPC) or Koopman MPC (KMPC). However, the Koopman-lifted states were derived from the physics behind wakes and turbine models. The controller highlighted in yellow utilizes autoencoder techniques and was developed by \cite{chen2022model}. The controllers highlighted in green are the proposed controllers in this work.

The table summarizes that the measurement requirements for designing the controller in AIC(AE1) are similar to those in our previous work, which also required fewer measurements compared to other existing literature. Moreover, AIC(AE2) necessitates even fewer measurements, solely relying on turbine power for identification and control.

%In this study, we aim to integrate Autoencoder and Koopman theory to identify two linear models without relying on expert knowledge and with limited measurements. That enables the real-time applicability of control schemes.
%Figure~\ref{fig:ModiAE} illustrates the block diagram depicting the integration of Koopman theory and autoencoder, denoted as the modified autoencoder. Unlike typical autoencoders where the encoder and decoder share similar activation functions, we employed linear activation for the decoder to learn the linear C matrix. Additionally, we introduced linear auxiliary networks (Anet and Bnet) between the encoder and decoder using the Koopman theory.
%The contribution of this paper lies in two folds by identifying two different models,
This study aims to integrate Autoencoder and Koopman theory to identify two linear models without expert knowledge and with limited measurements, enabling real-time applicability of control schemes. Unlike typical autoencoders, our modified autoencoder network (see fig.~\ref{fig:ModiAE} ) structure employs linear activation for the decoder to learn the linear $C$ matrix. Additionally, linear auxiliary networks (Anet and Bnet) are introduced using Koopman theory. We contribute by identifying two different models:
1) A modified autoencoder network structure that doesn't rely on expert knowledge for choosing Koopman-lifted states (referred to as Autoencoder model 2).
2)A modified autoencoder network structure and an efficient bilevel training algorithm, reducing the necessary measurements for identification and control. This reduction ensures the controller remains unaffected by measurement noise and changes in power coefficients due to aging (also referred to as autoencoder model 2).
 We compare the performance of control schemes using both identified models in three different scenarios: \begin{itemize}
    \item No measurement noise in wind speed measurements and no changes in power coefficients ($c_p$)
    \item Measurement noise in wind speed measurements and no changes in power coefficients ($c_p$)
    \item Measurement noise and changes in power coefficients
\end{itemize}
%Further, the comparison of the number of measurements required for identification and control in existing and proposed Koopman-based wind farm control is tabulated in Table ~\ref{tab:WFModels}.

%% The following sections will delve into the use of Autoencoders for system modeling and provide insights into various approaches and their limitations in different application domains.

% 1- Start with autoencoder to derive Koopman lifting functions (nature,sent email)\\
% 2- Autoencoder for wind farm control \cite{chen2022model} \\
% 3- Look from journal paper for introduction\\
% 4- Koopman with monomial, physically motivated \\
% 5- Comparison between our Koopman model obtained using physically motivated lifting function to Autoencoder\\

%6- Last para from problem formulation\\

 %In \cite{chen2022model}, a deep-learning-aided model predictive control method for wind farms considering the dynamic wake effect is proposed to control the learned wind farm reduced-order model which is identified by using autoencoder network. One of advantages of these methods is that both yaw angle and thrust coefficient are used to optimize wind farm power tracking performance in the model-based control system considering system constraints.


% Third possibility to calculate the $U_r$ is using power and power coefficients with the latter one are changing over time due to aging.
% In previously reported research the availability of grid of wind speed measurements points was assumed, e.g.$10^6$ measurement points in 3D grid for 2 turbines simulated in SOWFA and $14\times 10^3$ measurement points in 2D grid for 9 turbines simulated in WFSim \cite{chen2022model}. \cite{cassamo2021model}. In our previous work we relied on one wind speed measurement in front of the first turbine, the availability of correct power output of both turbines, and known power coefficients. We propose two different Autoencoder model \begin{itemize}
%     \item Autoencoder Model 1 : Effective wind speeds are estimated, and used as the scheduling parameters in qLMPC
%     \item Autoencoder Model 1 : WindFarm power is estimated, and used to design linear MPC
% \end{itemize}
% Remark: Model 1 uses similar approach as presented in our previous work with the difference that lifted functions are not based on physical knowledge. Model 2 is similar to our previous work in \cite{dittmer2023koopman}, however, the states are now based on individual turbine power rather than effective wind speed. We compare the performance of control schemes for three different scenerios: \begin{itemize}
%     \item No measurement noise in wind speed measurements and no changes in power coefficients ($c_p$)
%     \item Measurement noise in wind speed measurements and no changes in power coefficients ($c_p$)
%     \item Measurement noise and changes in power coefficients
% \end{itemize}
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/ModiAEKoopman.pdf}
    \caption{Identification of linear system representation of a nonlinear system by integrating Koopman and Autoencoder}
    \label{fig:ModiAE}
\end{figure}
% The active power control of wind farms is a challenging task due to aerodynamic interactions between turbines. Wake effects from upwind turbines can considerably reduce power yield from downwind turbines. Nevertheless, grouping turbines into farms has the advantage of optimizing the yield from favorable location and reduces maintenance cost per turbine.\\ 
% Wind farm control is hence a very active area of research. It has been demonstrated that both centralized, e.g. \cite{vali2019adjoint}, and decentralized, see \cite{marden2013model}, approaches have the potential to outperform currently used centralized, greedy control schemes, which do not take damage-equivalent loads or actuator energy into account. In the literature, two types of wake control have been described to minimize loads and maximize farm yield:\\
%\begin{enumerate} \item 
% For wake redirection control (WRC) upstream wind turbines are misaligned from incoming flow to deflect the wake so that downstream wind turbines are less affected by wakes. This can be achieved by tilting \cite{cutler2021optimization, fleming2014evaluating, fleming2015simulation}, yawing \cite{cassamo2021model} and individual pitch control \cite{frederik2020helix}.
% Axial induction control (AIC) varies generator torque and blade pitch angles from individual optimal setting to change the axial induction or thrust coefficient. In \cite{vali2019adjoint} and \cite{boersma2017tutorial} the two approaches are combined to maximize power output as well as reduce loads and actuator energy.\\
% %\end{enumerate}
% Two disadvantages of centralized schemes are the need for update rates within the millisecond range, below the typical wind turbine control update rate of 10 ms, as well as the necessity for information of wind turbine status including effective wind speeds acting on the rotor disk. Accurate wind measurements are in practice often unavailable.
% % which directly update the turbine controls,



%In literature several types of observers and neural networks have been such explored to estimate the effective rotor wind speed.

%In recent years, energy produced by wind turbines has increased exponentially.
% In practice, two independent PI loops for torque and pitch control are still widely used to maximize energy capture. 
%Wind turbine control is often implemented by two independent SISO PI control loops:  Torque or rotor speed control for below rated wind condition to maximize energy output and pitch control for above rated condition, keeping energy output constant and limiting loads.  Offline parameter optimization based on this classical PI approach, e.g. \cite{hoffmann2018load}, has been suggested as well as modern techniques, e.g. LQG, \cite{selvam2009feedback}, robust, \cite{basler2020genetic}, or repetitive control, \cite{liu2020adaptive}.
%Both linear and non-linear MPC have been applied to wind turbine control, NMPC motivated by non-linear dynamics in below rated condition, e.g. \cite{schlipf2013nonlinear, tofighi2015nonlinear}, and LMPC to reduce calculation time \cite{soliman2011multiple}.
%The models developed for simulations and for MPC in this work are parameterized with NREL 5MW research turbine parameters \cite{Jonkman2009} and compared to the widely used FAST environment \cite{jonkman2016fast}.
%In \cite{mulders2020preventing}  quasiLPV-MPC from \cite{cisneros2019wide} is applied to torque control for below rated wind. This paper focuses on the extension to the whole operating range, i.e. including above rated condition and pitch control, leveraging a velocity based algorithm \cite{cisneros2020velocity}.
%The advantages of this control scheme can be summarized as follows:
%\begin{enumerate}
%\item MPC allows effective control at different actuator rate and state constraints, of interest in scenarios with limited control action as described in \cite{liu2020adaptive}
%\item quasiLPV enables modelling faults and model uncertainties e.g. blade weight imbalance resulting in side-by-side motions for soft tower configuration, as discussed in \cite{mulders2020preventing}, or actuator fault, see \cite{adegas2012structured}
%\item velocity MPC alleviates the need for calculating and storing input and state operating point vectors \cite{cisneros2020velocity}.
%\end{enumerate}
%This paper is organized as follows: Section 2 presents the wind turbine model used as basis for the controller design. Section 3 gives a brief review of classical wind turbine control, and displays results obtained with a baseline controller for different models.  Section 4 describes the quasiLPV-MPC algorithm, followed by simulation results in section 5. Finally, a conclusion is provided in section 6.

%But for the last twenty years there has been research on load reduction leveraging both PI control as well as modern control designs. Offline controller tuning of PI parameters has been suggested: stochastic line search for multi-objective optimization \cite{hoffmann2018load} and Genetic Algorithms tuning of $H_{\infty}$ synthesis weights for controller designs taking into account modelling uncertainties \cite{basler2020genetic}. 

%Wind turbines need to operate as effectively as possible during their entire life time, which is typically around 20 years for onshore wind turbines 
%\begin{enumerate}
%\item the energy capture is to be maximized,
%\item such that the Operation and maintenance (O\&M) costs is kept as low as possible.
%\end{enumerate}
%Wind turbines need to operate as effectively i.e. the energy capture is to be maximized such that the Operation and maintenance (O\&M) costs is kept as low as possible.

%O\&M costs can be decreased by reducing the tower motions and rotor blades and hence decreasing the damage equivalent loads by using predictive, adaptive and fault tolerant control schemes. Various controller designs have been tested successfully, in simulation environments, but also on test benches and research wind turbines:
%\begin{enumerate}
%\item Offline controller tuning, e.g. stochastic line search for multi-objective optimization of PI parameters for IPC for load reduction \cite{hoffmann2018load} and Genetic Algorithms tuning of $H_{\infty}$ synthesis weights for controller designs taking into account modelling uncertainties \cite{basler2020genetic},
%\item Data-driven control designs, including iterative learning (ILC) \cite{liu2018spatial} and repetitive control \cite{liu2020adaptive},
%\item LQG design of IPC controller \cite{selvam2009feedback} %TODO other papers
%\item Linear and non-linear MPC: non-linear MPC based on LIDAR wind measurements \cite{schlipf2013nonlinear}
%\end{enumerate}

%Table \ref{tab:WFModels} is taken with some small modifications and additions from the theses \cite{smits2023fast} and \cite{adki2021MPC}. 

\begin{table*}[ht]
    \begin{center}
        \caption{Comparison of windfarm MPC schemes (related literature and proposed in this paper)}
        \label{tab:WFModels}
        \begin{tabular}{l l l l l l l l l} 
            \hline
            \hline
            Aspect & \cellcolor{blue!25}AIC\cite{boersma2018control} & \cellcolor{blue!25}WRC\cite{cassamo2021model}& \cellcolor{blue!10}AIC\cite{sharan2022real}& \cellcolor{blue!10}AIC\cite{dittmer2022data} & \cellcolor{blue!10}AIC+WRC\cite{dittmer2023koopman} & \cellcolor{yellow!25}AIC+WRC\cite{chen2022model} & \cellcolor{green!10}AIC (AE1) & \cellcolor{green!10}AIC (AE2) \\
            \hline
            $V_\infty$ speed & \cellcolor{blue!25}Constant & \cellcolor{blue!25}Constant & \cellcolor{blue!10}Constant  & \cellcolor{blue!10}Changing  & \cellcolor{blue!10}Constant & \cellcolor{yellow!25}Constant& \cellcolor{green!10}Constant & \cellcolor{green!10}Constant\\
          
             Turbines & \cellcolor{blue!25} 9 & \cellcolor{blue!25}2 & \cellcolor{blue!10}2  & \cellcolor{blue!10}2  & \cellcolor{blue!10}2 & \cellcolor{yellow!25}9 & \cellcolor{green!10}2 & \cellcolor{green!10}2\\
            \hline
            
            \textbf{Identification} & \cellcolor{blue!25}- & \cellcolor{blue!25}&\cellcolor{blue!10}& \cellcolor{blue!10} &  \cellcolor{blue!10} & \cellcolor{yellow!25}&  \cellcolor{green!10} & \cellcolor{green!10}\\
            Lifted states & \cellcolor{blue!25}- & \cellcolor{blue!25}$12,15,40...50$ &\cellcolor{blue!10}$6,12,24$ & \cellcolor{blue!10}$6$ &  \cellcolor{blue!10}$6$ & \cellcolor{yellow!25} $20$ &  \cellcolor{green!10} $20$ &\cellcolor{green!10} $2$ \\
            Input & \cellcolor{blue!25}- & \cellcolor{blue!25}$\gamma$ &\cellcolor{blue!10}$C_{T1}$, $C_{T2}$ &\cellcolor{blue!10}$C_{T1}$, $C_{T2}$, $V_1$  & \cellcolor{blue!10}$C_{T1}$,$C_{T2}$,$V_1$,$\gamma$ & \cellcolor{yellow!25}$C_{Ti}^{’}$, $\gamma_i$ $i= 1,2 ...9$ &\cellcolor{green!10} $C_{T1}$, $C_{T2}$ &\cellcolor{green!10} $C_{T1}$, $C_{T2}$  \\
            Output & \cellcolor{blue!25}-  & \cellcolor{blue!25}$P_{T1}$,$P_{T1}$  &\cellcolor{blue!10}$U_{r1}$ and $U_{r1}$ & \cellcolor{blue!10}$U_{r1}$ ,$U_{r1}$  &  \cellcolor{blue!10}$P_{WF}$ & \cellcolor{yellow!25}$P_{WF}$ &\cellcolor{green!10}$U_{r1}$ ,$U_{r1}$ &\cellcolor{green!10} $P_{WF}$ \\
            \hdashline
            &\cellcolor{blue!25} & \cellcolor{blue!25}& \cellcolor{blue!10}&\cellcolor{blue!10} & \cellcolor{blue!10} & \cellcolor{yellow!25} & \cellcolor{green!10} & \cellcolor{green!10} \\
            \multirow{-2}{5em}{Expert-Knowledge} & \multirow{-2}{*}{ \cellcolor{blue!25}- } &   \multirow{-2}{*}{\cellcolor{blue!25} not required} &\cellcolor{blue!10}\multirow{-2}{4em}{required}  & \cellcolor{blue!10}\multirow{-2}{4em}{required} & \cellcolor{blue!10}\multirow{-2}{4em}{required} & \cellcolor{yellow!25}\multirow{-2}{*}{not required} & \cellcolor{green!10} \multirow{-2}{*}{not required} & \cellcolor{green!10} \multirow{-2}{*}{not required}   \\
            \hdashline
            System Id & \cellcolor{blue!25}-  &  \cellcolor{blue!25}EDMD & \cellcolor{blue!10}EDMD & \cellcolor{blue!10}EDMD & \cellcolor{blue!10}EIODMD & \cellcolor{yellow!25} AE &  \cellcolor{green!10}AE+Koopman & \cellcolor{green!10} AE+Koopman  \\
            \hline
            \textbf{Control} &\cellcolor{blue!25}- &\cellcolor{blue!25}&\cellcolor{blue!10} & \cellcolor{blue!10}& \cellcolor{blue!10}& \cellcolor{yellow!25} &\cellcolor{green!10}& \cellcolor{green!10}\\
            \hdashline
             &\cellcolor{blue!25}- &\cellcolor{blue!25}&\cellcolor{blue!10} & \cellcolor{blue!10}& \cellcolor{blue!10}& \cellcolor{yellow!25} &\cellcolor{green!10}& \cellcolor{green!10}\\
              &\cellcolor{blue!25}- &\cellcolor{blue!25}&\cellcolor{blue!10} & \cellcolor{blue!10}& \cellcolor{blue!10}& \cellcolor{yellow!25} &\cellcolor{green!10}& \cellcolor{green!10}\\
           \multirow{-3}{6em}{Measurements} & \multirow{-3}{3em}{\cellcolor{blue!25}$P_{T1}$,$P_{T2}$, $U_{r1}$,$U_{r1}$ }&  \multirow{-3}{5em}{\cellcolor{blue!25}$10^6$points in 3D-grid, $P_{T1}$,$P_{T2}$}
                 & \multirow{-3}{6em}{\cellcolor{blue!10}$P_{T1}$,$P_{T2}$ } & \multirow{-3}{6em}{\cellcolor{blue!10}$P_{T1}$,$P_{T2}$, $V_1$ }  & \multirow{-3}{6em}{\cellcolor{blue!10}$P_{T1}$,$P_{T2}$, $V_1$ }& \multirow{-3}{6em}{\cellcolor{yellow!25}grid mesh $100\times 70$ } & \multirow{-3}{6em}{\cellcolor{green!10} $P_{T1}$,$P_{T2}$} & \multirow{-3}{6em}{\cellcolor{green!10} $P_{T1}$,$P_{T2}$}\\
               \hdashline
            Turbine Model & \cellcolor{blue!25}required & \cellcolor{blue!25}not required & \cellcolor{blue!10}required  & \cellcolor{blue!10}required  &  \cellcolor{blue!10}required  & \cellcolor{yellow!25}required & \cellcolor{green!10} required & \cellcolor{green!10} not required \\
            \hdashline
            &\cellcolor{blue!25} &\cellcolor{blue!25}&\cellcolor{blue!10} & \cellcolor{blue!10}& \cellcolor{blue!10}& \cellcolor{yellow!25} &\cellcolor{green!10}& \cellcolor{green!10}\\
              &\cellcolor{blue!25} &\cellcolor{blue!25}&\cellcolor{blue!10} & \cellcolor{blue!10}& \cellcolor{blue!10}& \cellcolor{yellow!25} &\cellcolor{green!10}& \cellcolor{green!10}\\
             \multirow{-3}{6em}{Controller} &\multirow{-3}{3em}{\cellcolor{blue!25}NMPC} &\multirow{3}{3em}{\cellcolor{blue!25}KMPC} & \multirow{-3}{3em}{\cellcolor{blue!10}qLMPC} & \multirow{-3}{5em}{\cellcolor{blue!10}online- adaptive qLMPC} &  \multirow{-3}{3em}{\cellcolor{blue!10}KMPC}  & \multirow{-3}{3em}{\cellcolor{yellow!25}NMPC}& \multirow{-3}{6em}{\cellcolor{green!10} qLMPC} & \multirow{-3}{6em}{\cellcolor{green!10}KMPC} \\
            
             \hdashline
            &\cellcolor{blue!25}  &\cellcolor{blue!25}  & \cellcolor{blue!10}  & \cellcolor{blue!10}  &  \cellcolor{blue!10}  & \cellcolor{yellow!25}  & \cellcolor{green!10}  & \cellcolor{green!10}\\
            \multirow{-2}{6em}{ Real-time capable} & \multirow{-2}{*}{ \cellcolor{blue!25}-} &  \multirow{-2}{*}{\cellcolor{blue!25}Yes } &  \multirow{-2}{*}{\cellcolor{blue!10}Yes } &  \multirow{-2}{*}{\cellcolor{blue!10}Yes } & \multirow{-2}{*}{\cellcolor{blue!10}Yes }&  \multirow{-2}{*}{\cellcolor{yellow!25}Yes } & \multirow{-2}{*}{\cellcolor{green!10}Yes } & \multirow{-2}{*}{\cellcolor{green!10}Yes } \\
              
             %  &\cellcolor{blue!25}  &\cellcolor{blue!25}  & \cellcolor{blue!10}  & \cellcolor{blue!10}  &  \cellcolor{blue!10}  & \cellcolor{green!25}\\
            % \hline
            % SOWFA  &  \multirow{3}{4em}{Fortran} & \multirow{3}{4em}{LES/3D-NSE}& \multirow{3}{4em}{High} & \multirow{2}{4em}{Order of hours to days}\\
            % PALM & & & &\\
            % EULAG  & & &  &\\
            \hline
             Software & \cellcolor{blue!25}WFSim & \cellcolor{blue!25}SOWFA & \cellcolor{blue!10}WFSim  & \cellcolor{blue!10}WFSim   & \cellcolor{blue!10}WFSim & \cellcolor{yellow!25}WFsim & {\cellcolor{green!10}WFsim } & {\cellcolor{green!10}WFsim } \\
             \hline
        \end{tabular}
    \end{center}
\end{table*}







==> 2ProblemFormulation.tex <==
\section{Problem Formulation}
Given a wind farm layout, a power grid reference $P_{ref}$, and free stream wind speed $V_{\infty}$, turbine control inputs, the thrust control signal $C'_T$ and yaw $\gamma$, are to be set such that power reference tracking error and the actuator activity are minimized subject to actuator limits and actuator rate constraints. In this work, we are comparing the performance of different centralized MPC schemes to optimize the controller signals for the wind farm layout depicted in figure \ref{fig:BlockDiagramFarm} which was also considered in \cite{sharan2022real,dittmer2022data}. The wind farm consists of two NREL 5MW wind turbines with a 5D (5$\times$ the rotor diameter) distance. The free stream is considered as constant with~8\,m/s, acting perpendicular on the first turbine. For more details see the turbine and farm layout provided in \cite{sharan2022real}. 
\begin{figure}[ht]
  \includegraphics[width=0.48\textwidth,trim={0 1cm 1cm 0},clip]{figures/drawBlockdaigram.pdf}
    \caption{Block diagram wind farm control}
    \label{fig:BlockDiagramFarm}
\end{figure}
A wind turbine can be represented as a quasi-linear parameter varying model (qLPV) \cite{dittmer2021velocity}, where the effective wind speed $U_{r}$ is the scheduling parameter. The effective wind speed of a turbine is defined as the mean of the wind speed components acting perpendicular to the rotor disk.
The first baseline control scheme considered in this work is the qLMPC \cite{boersma2018control} which uses the measurements of effective wind speeds ($U_{r\mathrm{i}}$) acting on the $\mathrm{i}^{\mathrm{th}}$ turbine respectively as scheduling parameters. 

 The effective wind speed at the second turbine is affected by wake, i.e., deficits in wind speeds at downwind turbines influenced both by free speed and control action of upwind turbines.
 Wakes, which are affected by factors like space, time, and various conditions, can be described using the Navier-Stokes equations. Wakes are causing slower wind speed, more turbulence, and wind direction changes \cite{boersma2017tutorial}.
Conventionally, these wakes are modeled using the Navier-Stokes equations (NSE):
\begin{align*} 
 \frac{\partial \bm{u}}{\partial t}+(\bm{u}\cdot \nabla_H)\bm{u}+\nabla_H\cdot\bm{\tau}_h+\nabla_H p-\bm{f} = 0,\quad  
\nabla_H\cdot \bm{u} =  \frac{\partial v}{\partial y}
\end{align*}
where $\bm{u} =[u \quad v]^T$ with $u$ and $v$ as wind components in $x$ and $y$ directions respectively, partial derivative $\nabla_H =[\partial/\partial x \quad \partial/\partial y]^T$ and $p = p(x,y,z_h)$ as a normalized pressure with air density $\rho$ at hub height ($z_h$). $\bm{\tau}_h$ is the subgrid stress tensor in horizontal direction of the turbulence model and $\bm{f}$ denotes the effect of turbines on the flow. 


  %To obtain $U_{r}$ for an individual turbine, solution of above mentioned NSE is required,for which no analytical solution is available. also the lots of measurements are required. 

The solution of the above-mentioned NSE can be used to obtain $U_r$ for an individual turbine. However, as no analytical solution exists, this can not be calculated in real-time. Measuring wind speeds at different grid points over a rotor disc can be done but requires expensive sensors, for example, spinner lidars \cite{mikkelsen2013spinner}. 

The second control scheme considered is our previously published Koopman-based qLMPC \cite{sharan2022real}, which uses Koopman models to estimate the effective wind speeds rather than assuming that the measurements are available. To identify the Koooman models, known physical relationships of the NSEs were exploited i.e, moving average of wind speed over an extended period, and the difference between current wind speeds to include the temporal and spacial wake components, as well as the cubic relationship between power and $U_r$.  

In this work, we want to investigate if we can get a similar or even better performance using no physical insight. Instead of designing Koopman lifted states via manually derived lifting function, lifted states are automatically set up using the integration of Autoencoder and Koopman framework.
We design two different Autoencoder models, 1) to estimate effective wind speeds 2) to estimate wind farm power. 
We compare the two baseline controllers and the two autoencoder-based controllers in three different scenarios: perfect wind speed measurements, degradation in wind measurements, and degraded wind measurement with an additional unnoticed change in the power coefficient.

%either the physical knowledge of the system was required or a lot of measurements were required. Different from the previous reported work this paper aims to design a purely data-driven control using an auto-encoder with very limited measurements.

==> Introduction.tex <==
\section{Introduction}
The active power control of wind farms is a challenging task due to aerodynamic interactions between turbines. Wake effects from upwind turbines can considerably reduce power yield from downwind turbines. Nevertheless, grouping turbines into farms has the advantage of optimizing the yield from favorable location and reduces maintenance cost per turbine.\\ 
Wind farm control is hence a very active area of research. It has been demonstrated that both centralized, e.g. \cite{vali2019adjoint}, and decentralized, see \cite{marden2013model}, approaches have the potential to outperform currently used centralized, greedy control schemes, which do not take damage-equivalent loads or actuator energy into account. In the literature, two types of wake control have been described to minimize loads and maximize farm yield:
\begin{enumerate}
        \item Wake redirection control (WRC): The upstream wind turbine is misaligned from incoming flow to deflect the wake so that downstream wind turbines are less affected by wakes. This can be achieved by tilting \cite{cutler2021optimization, fleming2014evaluating, fleming2015simulation}, yawing \cite{cassamo2021model} and using individual pitch control \cite{fleming2014evaluating, frederik2020helix}.
        \item Axial induction control (AIC): In this control strategy the generator torque and blade pitch angles are varied from individual optimal setting to change the axial induction or thrust coefficient. In \cite{vali2019adjoint} and \cite{boersma2017tutorial} the two approaches are combined to maximize power output as well as reduce loads and actuator energy.
\end{enumerate}
Two disadvantages of centralized schemes, which directly update the turbine controls, are the need for update rates within the millisecond range, below the typical wind turbine control update rate of 10 ms, as well as the necessity for information of wind turbine status including effective wind speeds acting on the rotor disk. Accurate wind measurements are in practice often unavailable.
\\
In this work, these issues are addressed by
\begin{enumerate}
\item using Koopman system identification for wind estimations removing the need for accurate wind measurements.
\item and reformulating an existing NMPC farm controller \cite{vali2019adjoint} by solving a QP, which reduces the controller update time from 30 to 4 ms,

\end{enumerate}
%
Recently, Koopman-based system identification for AIC and WRC for a wind farm of 2 turbines has been proposed in \cite{cassamo2021model, Cassamo.2020}, where input output DMD (IODMD) and extended input output DMD (EIODMD) were applied to get reduced order models.\\
In these proof-of-concepts, roughly hundred-thousand grid points from the high-fidelity simulation environment SOFWA have been considered for identification and validation. %These grid points were resampled from an original SOFWA grid of six million points that covered the three-dimensional space between two wind turbines with 505 points in lateral, 111 points in longitudinal and 99 points in vertical direction. 
The variance accounted for (VAF) of the power output of the Koopman model was shown to be more than 98\% for the first wind turbine and close to 90\% for the second turbine.\\
Based on the code and data from \cite{cassamo2021model}, we investigated that using only measurements obtained at the rotor disk at hub height similar levels of accuracy can be obtained. This makes IODMD applicable to real time data as well as to simulation data from WFSim which relies on 2D, rather than 3D Navier-Stokes, equations.\\
%made available at  https://github.com/nassircassamo/IODMD SOWFA, 
%In this paper, the koopman based ident\\ ified model is used to apply velocity-QLMPC AIC on wind farm of two turbines. Contribution of this paper is 1) Koopman-based model identification of wake only using effective rotor wind speed at each turbine (only two sample points).
%2) Velocity-QLMPC is applied to track the demanded power where the Koopman based wake model is used and reformulation of problem in quadratic programming shows the potential for real time applicability.
This paper gives an overview of Koopman theory in section \ref{KoopmanIdentification}. System identification results obtained with the  WFSim environment are provided in section \ref{WakeModel}. The MPC algorithm and its reformulation as a QP problem for real-time applicability are presented in section \ref{qLPMPC Design}. Closed-loop results based on the wind estimated using Koopman-based identified system are discussed in section \ref{SimResults}, and a conclusion is provided in section \ref{Conclusion}.
%In literature several types of observers and neural networks have been such explored to estimate the effective rotor wind speed.
\\
%In recent years, energy produced by wind turbines has increased exponentially.
% In practice, two independent PI loops for torque and pitch control are still widely used to maximize energy capture. 
%Wind turbine control is often implemented by two independent SISO PI control loops:  Torque or rotor speed control for below rated wind condition to maximize energy output and pitch control for above rated condition, keeping energy output constant and limiting loads.  Offline parameter optimization based on this classical PI approach, e.g. \cite{hoffmann2018load}, has been suggested as well as modern techniques, e.g. LQG, \cite{selvam2009feedback}, robust, \cite{basler2020genetic}, or repetitive control, \cite{liu2020adaptive}.
%Both linear and non-linear MPC have been applied to wind turbine control, NMPC motivated by non-linear dynamics in below rated condition, e.g. \cite{schlipf2013nonlinear, tofighi2015nonlinear}, and LMPC to reduce calculation time \cite{soliman2011multiple}.
%The models developed for simulations and for MPC in this work are parameterized with NREL 5MW research turbine parameters \cite{Jonkman2009} and compared to the widely used FAST environment \cite{jonkman2016fast}.
%In \cite{mulders2020preventing}  quasiLPV-MPC from \cite{cisneros2019wide} is applied to torque control for below rated wind. This paper focuses on the extension to the whole operating range, i.e. including above rated condition and pitch control, leveraging a velocity based algorithm \cite{cisneros2020velocity}.
%The advantages of this control scheme can be summarized as follows:
%\begin{enumerate}
%\item MPC allows effective control at different actuator rate and state constraints, of interest in scenarios with limited control action as described in \cite{liu2020adaptive}
%\item quasiLPV enables modelling faults and model uncertainties e.g. blade weight imbalance resulting in side-by-side motions for soft tower configuration, as discussed in \cite{mulders2020preventing}, or actuator fault, see \cite{adegas2012structured}
%\item velocity MPC alleviates the need for calculating and storing input and state operating point vectors \cite{cisneros2020velocity}.
%\end{enumerate}
%This paper is organized as follows: Section 2 presents the wind turbine model used as basis for the controller design. Section 3 gives a brief review of classical wind turbine control, and displays results obtained with a baseline controller for different models.  Section 4 describes the quasiLPV-MPC algorithm, followed by simulation results in section 5. Finally, a conclusion is provided in section 6.

%But for the last twenty years there has been research on load reduction leveraging both PI control as well as modern control designs. Offline controller tuning of PI parameters has been suggested: stochastic line search for multi-objective optimization \cite{hoffmann2018load} and Genetic Algorithms tuning of $H_{\infty}$ synthesis weights for controller designs taking into account modelling uncertainties \cite{basler2020genetic}. 

%Wind turbines need to operate as effectively as possible during their entire life time, which is typically around 20 years for onshore wind turbines 
%\begin{enumerate}
%\item the energy capture is to be maximized,
%\item such that the Operation and maintenance (O\&M) costs is kept as low as possible.
%\end{enumerate}
%Wind turbines need to operate as effectively i.e. the energy capture is to be maximized such that the Operation and maintenance (O\&M) costs is kept as low as possible.

%O\&M costs can be decreased by reducing the tower motions and rotor blades and hence decreasing the damage equivalent loads by using predictive, adaptive and fault tolerant control schemes. Various controller designs have been tested successfully, in simulation environments, but also on test benches and research wind turbines:
%\begin{enumerate}
%\item Offline controller tuning, e.g. stochastic line search for multi-objective optimization of PI parameters for IPC for load reduction \cite{hoffmann2018load} and Genetic Algorithms tuning of $H_{\infty}$ synthesis weights for controller designs taking into account modelling uncertainties \cite{basler2020genetic},
%\item Data-driven control designs, including iterative learning (ILC) \cite{liu2018spatial} and repetitive control \cite{liu2020adaptive},
%\item LQG design of IPC controller \cite{selvam2009feedback} %TODO other papers
%\item Linear and non-linear MPC: non-linear MPC based on LIDAR wind measurements \cite{schlipf2013nonlinear}
%\end{enumerate}
